SEMDR: A Semantic-Aware Dual Encoder Model for Legal Judgment Prediction with Legal Clue Tracing

Legal Judgment Prediction (LJP) aims to form legal judgments based on the criminal fact description. However, researchers struggle to classify confusing criminal cases, such as robbery and theft, which requires LJP models to distinguish the nuances between similar crimes. Existing methods usually design handcrafted features to pick up necessary semantic legal clues to make more accurate legal judgment predictions. In this paper, we propose a Semantic-Aware Dual Encoder Model (SEMDR), which designs a novel legal clue tracing mechanism to conduct fine-grained semantic reasoning between criminal facts and instruments. Our legal clue tracing mechanism is built from three reasoning levels: 1) Lexicon-Tracing, which aims to extract criminal facts from criminal descriptions; 2) Sentence Representation Learning, which contrastively trains language models to better represent confusing criminal facts; 3) Multi-Fact Reasoning, which builds a reasons graph to propagate semantic clues among fact nodes to capture the subtle difference among criminal facts. Our legal clue tracing mechanism helps SEMDR achieve state-of-the-art on the CAIL2018 dataset and shows its advance in few-shot scenarios. Our experiments show that SEMDR has a strong ability to learn more uniform and distinguished representations for criminal facts, which helps to make more accurate predictions on confusing criminal cases and reduces the model uncertainty during making judgments. All codes will be released via GitHub.

==> Tables/big_small.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\small
\centering
\begin{tabular}{l|cc|cc|cc|cc|cc|cc} 
\hline
Dataset                  & \multicolumn{6}{c|}{CAIL-small}                                                                        & \multicolumn{6}{c}{CAIL-big}                                                                                     \\ 
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Law Article} & \multicolumn{2}{c|}{Charges}    & \multicolumn{2}{c|}{Imprisonment} & \multicolumn{2}{c|}{Law Article} & \multicolumn{2}{c|}{Charges}    & \multicolumn{2}{c}{Imprisonment}            \\ 
\cline{2-13}
                         & MP             & F1              & MP             & F1             & MP             & F1               & MP             & F1              & MP             & F1             & MP             & F1                         \\ 
\hline
\texttt{TF-IDF+SVM}             & 78.68          & 73.89           & 79.04          & 75.16          & 36.71          & 31.93            & 84.56          & 77.10           & 82.64          & 75.14          & 50.13          & 50.14                      \\
\texttt{LSTM}                     & 79.99          & 78.43           & 81.81          & 81.07          & 39.61          & 33.96            & 84.70          & 84.61           & 85.41          & 84.43          & 41.29          & 38.32                      \\
\texttt{DPCNN}                    & 80.39          & 78.91           & 82.27          & 79.81          & 40.46          & 31.62            & 86.57          & 84.72           & 85.46          & 84.47          & 41.17          & 35.36                      \\
\texttt{NeurJudge$^+$}                & 80.99          & 79.86           & 83.28          & 81.71          & 36.43          & 35.33            & 89.28          & 87.04           & 92.12          & 89.66          & 40.35          & 38.17                      \\
\texttt{TextCNN}                  & 82.92          & 77.24           & 84.49          & 79.34          & 39.22          & 32.08            & 88.91          & 84.29           & 87.95          & 83.55          & 42.49          & 33.02                      \\
\texttt{TopJudge}                 & 82.59          & 77.72           & 79.71          & 75.31          & 32.42          & 31.49            & 85.41          & 80.59           & 85.67          & 81.16          & 36.80          & 34.68                      \\
\texttt{LADAN}                    & 84.95          & 78.79           & 82.90          & 82.84          & 34.69          & 35.62            & 90.01          & 90.08           & 87.81          & 88.86          & 50.97          & \multicolumn{1}{l}{51.77}  \\
\texttt{Few-Shot}         & 85.97          & 78.69           & 84.35          & 81.57          & 34.66          & 36.33            & 89.45          & 89.41           & 90.35          & 90.04          & 48.76          & 49.42                      \\
\texttt{BERT}                     & 89.20          & 88.97           & 89.66          & 89.49          & 44.60          & 41.05            & 95.82          & 95.44           & 96.37          & 96.47          & 54.96          & 54.67                      \\
\texttt{BERT-Crime}       & 89.64          & 89.15           & 90.01          & 90.44          & 44.78          & 41.14            & 96.07          & 95.58           & 96.65          & 96.49          & \textbf{55.20}         & 54.94                      \\ 
\hline
\textbf{\texttt{SEMDR}}           & \textbf{95.25} & \textbf{94.07}  & \textbf{93.59} & \textbf{94.86} & \textbf{44.94} & \textbf{43.98}   & \textbf{96.11} & \textbf{96.31}  & \textbf{96.81} & \textbf{96.64} & 55.16 & \textbf{55.42}             \\
\hline
\end{tabular}
}\caption{Legal Judgment Prediction in the High-Frequency Criminal Charge Scenario. SEMDR has tested three subtasks in the CAIL-small and CAIL-big datasets, which contain 121,045 and 1,520,744 criminal cases respectively.}
\label{tab2}
\end{table*}


==> Tables/instance.tex <==
\begin{table*}[!t]
\caption{Some Instances of Nodes and Relations in the Legal Judgment Reasoning Graph.}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{l|l} 
\hline
\textbf{Nodes/Relations}                      & \textbf{Instance}                                                                                                                                                                                \\ 
\hline
\multirow{3}{*}{Criminal Fact Node $(N_{F1})$} & Jack conspired with Tom and others (handled separately in other cases)...                                                                                                                        \\
                                    & to cheat the victim Joe out~of RMB 4000, a Bank of China card,~a Postal                                                                                                                          \\
                                    & \begin{tabular}[c]{@{}l@{}}Savings Bank card, a ring,~and keys, in the Postal Savings~Bank and Jack~ \\took out RMB 4000 from the bank card...\end{tabular}                                      \\ 
\hline
\multirow{2}{*}{Imprisonment Node $(N_{I})$}  & Three years of fixed-term imprisonment according to the Criminal Law of                                                                                                                          \\
                                    & the People's Republic of China...                                                                                                                                                                \\ 
\hline
\multirow{2}{*}{Charge Node $(N_{Ca})$}        & {[}Fraud] offenses involving significant amounts of public or private property~                                                                                                                  \\
                                    & \begin{tabular}[c]{@{}l@{}}shall be sentenced to up to~three~years in prison, detention, or control, and~\\may be fined; offenses involving large amounts or with other~serious...\end{tabular}  \\ 
\hline
\multirow{3}{*}{Law Article Node $(N_{A})$}   & [Article 266] stipulates that fraudulent appropriation of public or private property~                                                                                                             \\
                                    & of a significant amount~ can lead to imprisonment of up to 3 years,~with a fine                                                                                                                  \\
                                    & or singlepenalty. For a larger amount or other...                                                                                                                                                \\
\hline
Base\_article\_is Relation                    & Jack conspired with Tom... \textbf{Base article is}\textcolor[rgb]{1,0.643,0}{\textbf{~}}{[}Article 266] stipulates...                                                                           \\ 
\hline
Base\_charge\_is Relation                     & Jack conspired with Tom... \textbf{{Base charge is}}\textcolor{red}{~}{[}Fraud] offenses involving...                                                              \\ 
\hline
Base\_imprisonment\_is Relation               & Jack conspired with Tom... \textbf{Base imprisonment is} Three years of...                                                                                                                       \\ 
\hline
Be\_charged\_to Relation                      & {[}Article 266] stipulates... \textbf{Be charged to}\textcolor[rgb]{0,0.808,0.455}{\textbf{ }}{[}Fraud] offenses involving...                                                                    \\ 
\hline
Be\_sentenced\_to  Relation                   & Three years of... \textbf{Be sentenced to}\textcolor{red}{~}{[}Article 266] stipulates...                                                                                                        \\ 
\hline
Be\_imprisoned\_to Relation                   & {[}Fraud] offenses involving... \textbf{Be imprisoned to} Three years of...                                                                                                                      \\
\hline
\end{tabular}
}
\label{tab_ins}
\end{table*}

==> experiment.tex <==
% 修改意见V2:
% baseline部分的方法名称要加粗、黑体
% 从两个角度来阐述我们这么设计实验的一个目的
% 故事讲清楚、总分总形式、突出重点
% 图片大小需要注意
% 表达语言的书写方式
% 行文逻辑
% 我们做的工作突出是摆脱人工标记数据
% 修改意见V3:
% 最开始的工作集中在templet-base的方法
% 过渡到深度学习->自动化抽取信息
% 再到multi-task的形式抽取数据
% 再到随着大规模的预训练模型捕捉语义信号导致的“domain adaption”问题
% 回归提到uncertainty的问题(增加了文章的不确定性)
% 怎么通过sentence Representation进行语义增强
% 对比学习 现有语义信息 区分不同信息 细粒度(满足语义补充)
 \input{./Tables/dataset.tex}
 % 修改意见V4:
% t-sne的图像要更加准确直观 加上一个簇间分析、簇内分析
% case study要做的更多案例检索
 
In this section, the experimental settings of SEMDR and baseline models are described in detail. Basically, we conduct a series of experiments on three different scenarios: \textbf{high-frequency criminal charges}, \textbf{few-shot criminal charges} and \textbf{confusable criminal charges} selected from China Artificial Intelligence and Legal Challenges (CAIL2018). The experimental results are compared and analysed to verify the effectiveness of SEMDR.


\subsection{Experimental Datasets}
% Experimental
% The CAIL2018 is one of the publicly mainstream datasets and emplyed for most experiment in the research of LJP domain. For the SEMDR validation experiments, we have generated 5 datasets, namely CAIL-small, CAIL-big, Criminal-S,Criminal-M and Criminal-L, the former two of which aim to test the performance of SEMDR on the three sub-tasks of LJP in the general scenario, and the last three were used to specifically for testing accuracy on the criminal cases with confusing charges. \\
% 数据来源和筛选分开说
% 数据集和数据场景分开说
% \textit{Dataset Construction}. 
The dataset employed in our experiments is from the public dataset of CAIL2018, which contains the practice stage of data (CAIL-small), and the competition stage of data (CAIL-big). Besides, we have specifically selected cases from the CAIL dataset that are highly confusing or have a low frequency of occurrence to form the CAIL-mixed. Statistics for these datasets are listed in table \ref{tab:1}, with reference to data filtering techniques for existing works ~\cite{zhong-etal-2018-legal}, and we concentrate only on criminal cases with a single judgment.
% 老版本的small和big
% \input{./Tables/cail_small.tex}
% \input{./Tables/cail_big.tex}
% 新版版的small和big
\input{Tables/big_small.tex}
\subsection{Baselines}
We utilize several typical text classification models and neural network prediction models as baselines:

\texttt{TF-IDF+SVM}: Term-frequency Inverse Document Frequency (TF-IDF) is a statistical method used to evaluate the importance of a word in a document set and Support Vector Machine (SVM) is employed for classification.
 
\texttt{LSTM}: Long Short-Term Memory (LSTM) performs better in longer sequences than traditional Recurrent Neural Network (RNN) models. LSTM utilizes forget gate, input gate and output gate to deal with gradient disappearance and gradient explosion during a long training sequence.
 
\texttt{TextCNN}: TextCNN is similar to Convolutional Neural Network (CNN) in computer vision. The most significant difference between traditional CNN and TextCNN is the input data, where TextCNN inherits the advantages of CNN.
% Due to parameter sharing, it can achieve high performance with fewer parameters.

\texttt{DPCNN}: Deep Pyramid Convolutional Neural Networks (DPCNN) is developed for Text Categorization, which can extract long-distance text dependency through deepening the network. DPCNN leverages region embedding, convolution kernel and residual-connection to build the deep model. 
% In a strict sense, DPCNN is the first word-level widely effective CNN for deep text classification.

\texttt{BERT}: Bidirectional Encoder Representations from Transformers (BERT) uses multiple encoders of Transformer and it can capture bidirectional context information. BERT is fully pre-trained in large-scale corpus through a masked language model. 
% BERT has a large number of parameters and it has achieved the best results in several different NLP tasks. 
% In our experiments, pre-trained BERT on Chinese corpus is employed.

\texttt{TopJudge}: TopJudge is a unified framework, which can deal with multiple LJP subtasks through topological learning on Directed Acyclic Graph.

\texttt{Legal Attributes}:  Legal Attributes is the first multi-task model specifically designed to predict few-shot charges and confusing charges. In addition, annotated legal attributes of charges have been combined to enhance the keywords information in the criminal fact representation.  

\texttt{NeurJudge}: NeurJudge uses the predicted results of intermediate subtasks to divide factual descriptions into different situations and uses them to make predictions about other subtasks.  

\input{./Tables/results_s2s3.tex}
\subsection{Scenarios Description}
% \textbf{Scenarios Description.} 
% High-Frequency Criminal Charge Scenario \textbf{(Scenario I)}. We define a criminal charge as the high-frequency category accusation if it has ${\ge}$ 100 occurrences and its related articles have ${\ge}$ 10 cases in the dataset. 
Based on the frequencies of Legal Judgment Prediction (LJP) shown in CAIL dataset, we have defined 3 scenarios: \textt{high-frequency charge scenario}, \textt{few-shot charge scenario} and \textt{confusable charge scenario}.

Specifically, the high-frequency criminal charge scenario contains criminal charges that have more than 100 cases while maintaining over 10 frequencies of law articles in CAIL-small and CAIL-big. 

To confirm that SEMDR has good classification ability even for uncommon or low-probability of crime types, we also have collected criminal cases whose frequencies are between ${\ge} $ 50 and ${\leq}$ 100 to form the few-shot criminal charge scenario.

In addition, we select 10 criminal charges that could easily be misjudged against each other to develop the confusable accusation scenarios (including: \textt{confuse-small, confuse-medium and confuse-large}) where there are 50,000 cases, 75,000 cases and 100,000 cases respectively.

\subsection{Implement Details}
% \textbf{Experimental Settings.} 
For the division of the dataset, we reserve roughly 80\% of the selected cases as the training set in all scenarios, and the rest is equally separated into the validation and test parts. 
% SimCSE as a 
In the clue-aware continuous learning model, given that fact description are in Chinese, we apply Bert-base-Chinese as the pre-train language model combined with a constructive learning strategy to generate the corresponding 256-dimensional representation. In the legal judgment reasoning graph, we train 5000 epochs for a 2-layer Graph Attention Network (GAT) with a multi-head mechanism to aggregate connected fact nodes and legal judgment nodes.

For the models in baseline, we used THULAC for word segmentation, which is excellent in handling Chinese segmentation. More details in the CNN-based comparison models, we set the maximum document length to 256, while for the RNN-based comparison models, we set the maximum number of words in a sentence to 150 and the maximum number of sentences in a document to 15. Based on the preliminary experimental results on evaluation tests, we used the Adam optimizer with a learning rate of 0.01 and set the dropout to 0.5. 

\textit{Evaluation Metrics.}
We employ accuracy (Acc), macro-precision (MP), macro-recall (MR) and macro-F1 (F1) as evaluation metrics.

\subsection{Overall Performance}
% SEMDR 模型比所有baseline模型都要好, 相比于机械模型都要好.LSTM-based比较的话，指标有显著的好，跟其中的topjudge相比有10%的提升，跟基于预训练模型的方法也保持了一致的提升. 说明了SEMDR建立语义图非常有效地强化了了sentence Representation学习，进一步更好地提升预测准确性。
% 分成两部分来说，small来讲，SEMDR相比较bert有很好的效果，这样显著的效果体现了模型有更好的few-shot的能力.
We evaluate our model's and baselines' results on three LJP subtasks and find that SEMDR has beaten the others to achieve state-of-the-art performance. Through the experimental results shown in Table \ref{tab2}, SEMDR is much better than all mechanical models and has significantly improved LSTM-based models' performance. Notably, there is roughly a 10\% improvement compared to the TopJudge, one of the best LJP-based LSTM models. SEMDR also maintains a consistent improvement compared to the pre-trained model-based approaches. It further indicates that SEMDR builds semantic graphs that are very effective in enhancing the learning of sentence representation and improving prediction accuracy.

Moreover, as shown in Table \ref{tab3}, SEMDR is more sensitive and has obtained better prediction results compared to BERT to in the few-shot criminal charge scenario and confusable criminal charge scenario. The significant improvement reflect our model has superior ability to solve LJP tasks in different scenarios.
% In general, through the experimental results shown in Table \ref{tab2} and \ref{tab3}, we can find that our model achieves better results on most of the evaluation metrics in all LJP subtasks, especially in the task of law article prediction and legal accusation prediction.

% As we compare the results of SEMDR in 3 different application scenarios, our model is more sensitive to the few-shot criminal charge scenario and confusable criminal charge scenario, and the accuracy (Acc) has been improved over 2.1\% in both situations. We have compared our model with baseline models in 3 different confusable accusation datasets, where SEMDR exceeds other baselines significantly on the confuse-large.

% 时间轴线: 05:14-08:05
% 第一段什么是few-shot 什么是confuse，S M L 以及怎么划分
% 和confuse的区别，以及划分成三个场景的，以及三者的目的
% 分析：从基线上比, TopJudge 和 Legal Attributeb和BERT的区别是lstm 但是比bert好.BERT不是万能的
% SEMDR模型可以显著提升BERT
%第三段:
% 有一个非常稳定和稳步的提升，
% 不管数据集是sml三种，说明这样一个好的现象可以利用有限的知识显著提升
\subsection{Performance on Different Scenarios}
% For the high-frequency criminal charge scenario in CAIL-small and CAIL-big, SEMDR exceeds the text classification models in both datasets. Its accuracy improves as the training set increases, confirming that case aggregation enhances the comprehension of LJP nodes in the legal judgment reasoning graph. In addition, it is worth noting that the prediction in terms of penalty is not stable, which can be summarized into two main reasons. The first one is the distribution of imprisonment is more random than charges and law articles, and the other reason is the short and similar semantic description content in each legal imprisonment node.
We have simulated 3 criminal scenarios to verify that SEMDR has excellent and stable prediction performance in different criminal charges. Specifically, the high-frequency charge scenario contains criminal charges have more than 100 cases and over 10 frequencies of law articles; The few-shot charge scenario collects criminal cases with frequencies in 50 to 100; In addition, we select 10 criminal charges that are prone to misjudgment to fill the confusing charge scenario and divide them sequentially confuse-small, confuse-medium and confuse-large according to the size of the cases.

For the high-frequency criminal charge scenario in CAIL-small and CAIL-big, SEMDR exceeds the text classification models in both datasets. Its accuracy improves as the training set increases, confirming that case aggregation enhances the comprehension of LJP nodes in the legal judgment reasoning graph. In addition, the prediction of law imprisonment could be more stable, which can be concluded into two main reasons. The first one is the distribution of terms of penalty is more random than charges and law articles, and the other reason is the short and similar semantic description content in each law imprisonment node.

For the few-shot criminal charge scenario in CAIL-mixed, as shown in Table \ref{tab3}, we can intuitively find the accuracy of SEMDR and other baseline models both is less than 60\% due to insufficient training in criminal cases. Nevertheless, when we analyze these results in a longitudinal direction, there was an over 2.1\% improvement in the task of law charge prediction. Thus we find SEMDR's performance is greatly enhanced as the number of relevant criminal cases increases.

For the confusable criminal charge scenario, when we concentrate on the ten confusing accusations, our model's ability to identify them gradually increases and stays above 94\% with slight fluctuations, which is ahead of the other models compared and about 2\% higher than the best baseline model. As shown in Table \ref{tab3}, we can conclude that reasoning more relevant criminal cases can effectively solve the problem of misjudgment among confused criminal charges.

\input{./Tables/AS2.tex}
% \begin{figure}[t]{
%  \subfigure[\label{fig:3a}Average Distance.]{
%             \includegraphics[width=0.23\textwidth]{./Figures/new_vis_3_type_average_distance.pdf}
%             }
%     % \hspace{1pt}
%      \subfigure[\label{fig:3b}Attention Entropy.]{
%            \includegraphics[width=0.21\textwidth]{./Figures/new_vis_3_type_average_entropy.pdf}
%             }
%     \caption{\label{fig:3}The average distance and attention entropy between legal charges and corresponding criminal cases in the confusable criminal charge scenario.}
%     }
% \end{figure}
% 时间轴12:45-13:58
%问题是写的内容是反着写的
%长文本的处理是hardcore非常难的一件事，加入了clues tracing之后，有了5%的提升，这样显著的提升体现ctracing可在保留更多法律信息的基础上以对文章进一步的简化
% 在保留更多法律信息的基础上，可以以此来解决法律领域长文本的表示问题
% accuracy was maintained at 60\% to 65\% for law article prediction and charges prediction. While the worst performance is the prediction of imprisonment, which is under 16\%.
\subsection{Ablation Study}
% 16:40-16:
% 第一段先总写,我们有三个模块，分别验证了在模型中的role.三个模块分别去介绍,细致一点来讲哪个部分是最有用的，我们发现基于图的case enhangcement最后，相同的case聚合，不同的case在对比学习的时候进行一个训练，达到了一个最好得效果，
Our model has 3 modules: clue tracing, contrastive learning and case enhancement. This subsection conducts an ablation study to investigate the roles played by each module in SEMDR.
The performance in Table \ref{tab4} shows that all the modules can modify prediction accuracy. Nevertheless, we also can observe that the case enhancement module has achieved the most remarkable improvement as ($\mathbf{\uparrow} \textbf{27.79\%}$). During the case enhancement on the legal judgment reasoning graph, we aggregate the criminal cases with the same judgments, consequently achieving the best results. In addition, we also carry out clue tracing and contrastive learning for advanced criminal case representation.
% As shown in Table 5, SEMDR is characterized by incorporating three semantic-aware encoder components in the Legal Judgment Prediction (LJP). Thus, we have designed corresponding ablation experiments to test the influence of each module on prediction accuracy. 
% We first use the BERT model to embed the text data, then obtain the vectors of crime facts and legal texts separately and calculate the legal judgment with the highest association (dot product) as the prediction result. 

% The performance of SEMDR in Table \ref{tab4} shows that prediction accuracy was maintained at 60\% to 65\% for law article prediction 
% and charges prediction.
% By contrast, the worst performance is in the prediction of imprisonment, which is under 16\%.
% 除此之外，我们对于criminal case我们可以进行clues-tracing 和对比学习，然后在总分
% 时间轴12:45-13:58
%问题是写的内容是反着写的
%长文本的处理是hardcore非常难的一件事，加入了clues tracing之后，有了5%的提升，这样显著的提升体现ctracing可在保留更多法律信息的基础上以对文章进一步证明文章的有效性
% 在保留更多法律信息的基础上，可以以此来解决法律领域长文本的表示问题
Although processing long documents is a hardcore task, SEMDR achieved a significant 5\% improvement in results after adding the clue-tracing module, which reflects that the clue-tracing method can further prove the validity of our model based on retaining more legal information.
% Due to the large size of the judgment document, it is challenging to analyze the full-text, especially in confusing legal charges requiring strict boundary separation. We consequently apply a fine-grained method to extract criminal clues, and the accuracy of SEMDR generally rises by more than 5\%.

Another significant increase in SEMDR comes from the contrastive learning module. Similar of using positive and negative samples in supervised learning in SimCSE, we define a contrast crime pair for each criminal fact based on whether the verdict is the same or not.
% we first remove the fine-grained method of tracing criminal clues and use the traditional full-text analysis method to extract core clues. The results in Table 5 show that the prediction accuracy decreases by more than 10\%. Then we removed the contrastive learning model of SEMDR to analyse the impact of a semantic-aware pre-trained language model on the representation of unknown fact description.

% 最后三个模块cooperation协同起到了作用
% cooperation s三个模块的
In conclusion, the above three modules cooperate to achieve dramatic ($\mathbf{\uparrow} \textbf{35.26\%}$) overall improvement, which further proves the effectiveness of SEMDR in LJP tasks.
% The final element to be analyzed is the algorithm of criminal case enhancement in the legal judgment reasoning graph. We can observe that the performance has increased dramatically ($\mathbf{\uparrow} \textbf{35.26\%}$). The above results claim that the fine-grained clue tracing and semantic enhancement of relevant crimes are two core factors affecting prediction accuracy.
% 2022、11、10之前的版本
% The final element to be analysed is the algorithm of criminal case aggregation in the legal judgment reasoning graph. We eliminate the node training pattern of the graph attention network (GAT). We can observe that the performance has increased greatly ($\mathbb{\uparrow} \mathbf{27.79\%}$). From the above results, we can conclude that the two core factors affecting prediction accuracy are fine-grained criminal clues and semantic enhancement of relevant crimes. Thus, it verifies our claim that the relevant case aggregation approach can effectively improve the SEMDR model's ability to predict unknown cases in the legal judgment reasoning graph.
% 2022.11.10之前的版本
% From the above results, we can conclude that fine-grained criminal clues and semantic enhancement of relevant crimes are the two core factors affecting prediction accuracy. Thus, it verifies our claim that the relevant case aggregation approach can effectively improve the SEMDR model's ability to predict unknown cases in the legal judgment reasoning graph.
% \input{./Tables/AS.tex}
% \input{./Tables/AS2.tex}
% \input{./Tables/results_s2s3.tex}
% our ablation tests are conducted in the Scenario I (CAIL-small) and the experiment results are shown in Table 7. We can observe that the performance has dropped greatly as we replace any component of SEMDR, especially the method of semantic enhancement on criminal cases. Nearly 30\% decline in all metrics reveals that GAT is a efficient pattern to trace the criminal clues and then improve the ability to identify confusing accusation. 
% 图重新画
% \begin{figure}[t]        
%     \centering
%      \includegraphics[width = 1\linewidth] {./Figures/t-SNE_V3.pdf}    
%     \caption{\label{3}Embedding Visualization (t-SNE) of Different Criminal Facts. The ${``\bullet"}$ in different colours denotes the criminal fact embedding of theft, robbery and fraud respectively. The aggregation process in the inference diagram is shown sequentially from Figure 3(a) to 3(d).} 
% \end{figure}
% \begin{figure}[t]
% \centering
% \subfigure{
% \begin{minipage}[t]{0.45\linewidth}
% \centering
% \begin{mdframed}
% \includegraphics[width=1in]{./Figures/0.pdf}
% \end{mdframed}
% \caption{Original Distribution}\label{fig:7a}
% \end{minipage}%
% }%
% % \end{subfigure}
% \quad
% \subfigure{
% \begin{minipage}[t]{0.45\linewidth}
% \centering
% \begin{mdframed}
% \includegraphics[width=1in]{./Figures/100.pdf}
% \end{mdframed}
% \caption{100 Epochs}
% \end{minipage}%
% }%
% \quad
% \subfigure{
% \begin{minipage}[t]{0.45\linewidth}
% \centering
% \begin{mdframed}
% \includegraphics[width=1in]{./Figures/500.pdf}
% \end{mdframed}
% \caption{500 Epochs}
% \end{minipage}%
% }%
% \quad
% \subfigure{
% \begin{minipage}[t]{0.45\linewidth}
% \centering
% \begin{mdframed}
% \includegraphics[width=1in]{./Figures/1000.pdf}
% \end{mdframed}
% \caption{1000 Epochs}
% \end{minipage}%
% }%
% \centering
% \caption{Embedding Visualization (t-SNE) of Different Criminal Facts. The ${``\bullet"}$ in different colours denotes the criminal fact embedding of theft, robbery and fraud respectively. The aggregation process in the inference diagram is shown sequentially from Figure 3(a) to 3(d).}\label{fig:7}
% \end{figure}
% 更改t-sne图片
% 加一个 不做clues tracing的
% 合道一起的图片
% \begin{figure}
%   \centering
%   \includegraphics[scale=0.5]{./Figures/new_vis_3_type_average_distance.pdf}
%   \hspace{1in}
%   \includegraphics[scale=0.5]{./Figures/new_vis_3_type_average_entropy.pdf}
%   \caption{test}
% \end{figure}
% 合道一起的图片
\begin{figure}[t]{
     \subfigure[\label{fig:3b}Cross-Entropy.]{
           \includegraphics[width=0.45\linewidth]{./Figures/new_vis_3_type_average_entropy_v2.pdf}
            }
             % \hspace{1pt}
 \subfigure[\label{fig:3a}Average Distance.]{
            \includegraphics[width=0.45\linewidth]{./Figures/new_vis_3_type_average_distance_v2.pdf}
            }
    }
    \caption{\label{fig:3}The cross-entropy and average distance between legal charges and corresponding criminal cases in the confusable charge scenario.} 
\end{figure}
% ps直接合并
% \begin{figure}[t]        
%     \centering
%      \includegraphics[width = 1\linewidth] {./Figures/kk.pdf}    
%     \caption{\label{fig:3}The cross-entropy and average distance between legal charges and corresponding criminal cases in the confusable criminal charge scenario.} 
% \end{figure}
\begin{figure}[t]{
      \subfigure[\label{fig:4a}Distribution of Legal Accusations and Corresponding Cases after BERT Embedding.]{ 
            \includegraphics[width=0.222\textwidth]{./Figures/new_vis_3_edu_v3_1.pdf}
            }
  \hspace{1pt}
     \subfigure[\label{fig:4b}Distribution of Legal Accusations and Corresponding Cases after SEMDR.]{
            \includegraphics[width=0.222\textwidth]{./Figures/new_vis_3_edu_v3_3.pdf}
            } 
    \caption{Embedding visualization (t-SNE) of different criminal facts. The $``\;\rule[0.1em]{0.4em}{0.40em}\;"$ in different colours denotes the legal charges embedding of \textbf{<{\color{orange} robbery} , {\color{blue} theft} , {\color{purple}{fraud}}>} respectively and the ${``\bullet"}$ represents the fact embedding of their criminal cases. Figure \ref{fig:4a} to \ref{fig:4b} demonstrates the distribution of criminal cases and legal charges after different modules in SEMDR.}
    }
\end{figure}
% 结合数据进行定量分析
% \begin{figure}[t!]        
%     \centering
%     % \lefting
%     \includegraphics[width = 0.5\textwidth] {./Figures/attention_charges_cases.pdf} 
%     \caption{\label{1}Association score among 3 confusable charges and their corresponding cases. X-axis and y-axis denote criminal cases and law charges respectively.} 
% \end{figure}
% clues_tracing.pdf
\subsection{Embedding Visualization with SEMDR}
This subsection visualizes the embedding of criminal facts and legal judgment in SEMDR model and further explores the different modules' guidance through their spatial distribution.
The SEMDR's performance in confusable criminal charges scenario is shown in Figure \ref{fig:3}. We observed that the average distance between charges and their cases decreased nearly ${44\%}$ from Figure \ref{fig:3a}. The distinction between charges embedding is enhanced as the number of training epochs increases. Meanwhile, the reasoning graph can fuse the relevant cases as extra features during training, which further reduces the distance between criminal cases. According to the results in Figure \ref{fig:3b}, the value of cross-entropy decreases with each individual module, with lower cross-entropy standing a more homogeneous and stable distribution.

Moreover, we choose 3 typical confusable criminal charges (${<\textbf{robbery, theft, fraud}>}$) and randomly sample 5 existing cases belonging to each charge. The t-SNE~\cite{van2008visualizing} is employed to visualize the original embedding distribution of accusations and their cases.
Figure \ref{fig:4a} illustrates the chaotic and disordered distribution of BERT embedding. One notable point is that the boundary between the 3 confusable charges is highly ambiguous but case nodes and charge nodes are significantly apart.
This disparate separation between criminal cases and legal charges indicates their weak association.
As shown in Figure \ref{fig:4b}, it is intuitive to notice both clues-aware continuous learning and case enhancement can strengthen the interpretation of legal provisions in cases. Specifically, the similarity between different charges has been greatly suppressed, and their cases are gradually clustering with the corresponding charges.
% Specifically, the distance between offences becomes significantly larger and the similarity between the legal provisions of accusations is significantly suppressed.
% According to the results in the Figure 3(d), the distinction between confusable accusation embedding is enhanced, specifically the distance between offences becomes significantly larger and the similarity between the legal provisions of accusations is significantly suppressed.
% Distance of different crimes. According to the results in the Figure 3(d), the similarity between the legal provisions of accusations 
% The distinction between confusable accusation embedding is enhanced, specifically the distance between offences becomes significantly larger and the similarity between the legal provisions of accusations is significantly suppressed.
% Then we choose 3 typical confusable criminal charges(${<\textbf{Theft, Robbery, Fraud}>}$) and randomly sample 5 existing cases of each from CAIL-mixed. Figure 3 demonstrates the training process for criminal cases in SEMDR. 
% Before training starts, we first employ t-SNE~\cite{van2008visualizing} to visualize the original criminal embedding of these accusations.
% \begin{figure}[t]{
%       \subfigure[Distribution of legal accusations and corresponding cases after BERT embedding.]{ 
%             \includegraphics[width=0.85in]{./Figures/rawbert_vis_3_edu.pdf}
%             }
%     \hspace{5pt}
%      \subfigure[Distribution of legal accusations and corresponding cases after clues-aware continuous learning.]{
%             \includegraphics[width=0.85in]{./Figures/2f.pdf}
%             }
%             \hspace{5pt}
%      \subfigure[Distribution of legal accusations and corresponding cases after 5000-time case aggregation.]{
%             \includegraphics[width=0.85in]{./Figures/3f.pdf}
%             }
%             % \hspace{10pt}
%      \subfigure[Distance between each of
% two legal accusations in <robbery, theft, fraud>.
% ]{
%             \includegraphics[width=1.35in]{./Figures/3fe3.png}
%             }
%                     \hspace{1pt}
%      \subfigure[Distance between each of legal accusations and corresponding criminal cases.
% ]{
%           \includegraphics[width=1.35in]{./Figures/3fd3.png}
%             }
% %  \end{mdframed}
%     \caption{Embedding Visualization (t-SNE) of different criminal facts. The $``\;\rule[0.1em]{0.4em}{0.40em}\;"$ in different colours denotes the legal accusation embedding of robbery, theft and fraud respectively and the ${``\bullet"}$ represents the criminal fact embedding of their cases.}
%     }
%     % The aggregation process in the inference diagram is shown sequentially from Figure 3(a) to 3(c).
% \end{figure}
% When the training times exceed 1000, we observe that the spatial vectors of some cases in the graph are identical and overlap in the graph, and the inter-class distances of the charges expand further significantly.
% \begin{figure} [t]  
%     \centering
%     \includegraphics[width = 1\linewidth] {./Figures/v8.pdf}
%     \caption{\label{3} An example case easily misjudged and its legal judgment prediction by different models.}
% \end{figure}
% 结合图像进行定性分析
% case study的图放入附录
% 调研baseline
% attention_charges_cases_v4.pdf
% \begin{figure} [t]  
%     \centering
%     \includegraphics[width = 1\linewidth] {./Figures/Project description of historical data Version2.7.pdf}
%     \caption{\label{3} An easily misjudged criminal case and its legal judgment prediction by different models.}
% \end{figure}
\begin{figure}[t]{
 \subfigure[\label{fig:6a}The Association between the Charge of Robbery with the Description of Motivation and Action.]{
            \includegraphics[width = 1\linewidth]{./Figures/clues_tracing_v3.pdf}
            }
    % \space{1pt}
  \subfigure[\label{fig:6b}Coverage between the Confusable Charges with Some Keywords in the Fact Description.]{
           \includegraphics[width = 1\linewidth] {./Figures/case_study_v6.pdf}
            }
    \caption{\label{fig:6}An attention heatmap of a robbery case with different candidate charges.}
    }
\end{figure}
%印证model uncertainty的
\begin{figure} [t]  
    \centering
    \includegraphics[width = 1\linewidth] {./Figures/case study v3.pdf}
    \caption{\label{fig:6a}The Association between the Charge of Robbery with the Description of Motivation and Action.}
\end{figure}
% \begin{figure}[t]{
%  \subfigure[\label{fig:6a}The Association between the Charge of Robbery with the Description of Motivation and Action.]{
%             \includegraphics[width = 1\linewidth]{./Figures/case_study_v10.pdf}
%             }
%     % \space{1pt}
%   \subfigure[\label{fig:6b}Coverage between the Confusable Charges with Some Keywords in the Fact Description.]{
%            \includegraphics[width = 1\linewidth] {./Figures/case_study_v6.pdf}
%             }
%     \caption{\label{fig:6}An attention heatmap of a robbery case with different candidate charges.}
%     }
% \end{figure}
\subsection{Contributions of Clue Chains}
This subsection further demonstrates how the chain of clues in SEMDR can logically reason and accurately predict in a(n) robbery (error-prone) case.
% research the contribution of legal judgment reasoning graph semantics by investigating the  association score learned on the different types of legal charges.

\textit{Contributions of Clues-Tracing.} Filtering out redundant attributes in criminal fact description, such as personal privates, location, time, and so on, thereby concentrating additional on legal cues (i.e., motivation, action, and harm), ensures SEMDR to avoid unjust judgment due to the coincidence of these factors. As shown in Figure \ref{fig:5}, the analysis of the full text gives incorrect predictions, showing the highest correlation with theft (${37.8\%}$), not robbery (${30.1\%}$), and a strong correlation with fraud (${28.6\%}$) because the descriptions of the crimes included many descriptions of money transactions. Conversely, in Figure \ref{fig:6a}, the clues-tracing module can predict the correct charge, robbery (${88.0\%}$), then be combined with a comparative learning approach to highlight the weight of motivation (${21.0\%}$) and action (${63.0\%}$) in the fact description.

% local trap局部陷阱
\textit{Contributions of Cases Enhancement.} One of the great difficulties in identifying confusable cases is falling into the trap of some local similarity but ignoring the global balance. As shown in Figure \ref{fig:6b}, the criminal behaviors are similar to the cash transaction process in fraud, and the loss of property in harm will be confused with theft. However, the transaction is based on a compulsory sale that should be legally nonexistent. In this situation, it should be the robbery and not the other two charges. To summarize, SEMDR can extend the training range with the guidance of fine-grained analysis of legal clues, and the reasoning of the case enhancement can significantly help LJP models to solve ambiguous crime predictions.
% One of the great difficulties in identifying confusable cases is falling into the trap of some local similarity but ignoring the global analysis. As shown in Figure \ref{fig:7}, the criminal behaviors are similar to the cash transaction process in fraud, and the loss of property in harm will be confused with theft. However, the transaction is based on a forced sale that should be legally nonexistent. In this situation, it is a robbery case and not the other two charges. To summarize, SEMDR can extend the training range and provides the correct answer with the guidance of fine-grained analysis of legal clues, and the reasoning the related criminal cases can significantly help LJP models to solve the problem of predicting conflict.
% The contribution of each individual criminal case enhancement in SEMDR is shown in Figure \ref{fig:5}. The weight of three confusable charges (${<\textbf{Robbery, Theft, Fraud}>}$) is almost significantly distinct distribution, indicating the effectiveness of entities and all components are important in SEMDR.

% \begin{figure} [t]   
%     \centering
%     \includegraphics[width = 1\linewidth] {./Figures/case_study_v8.pdf}
%     \caption{\label{fig:6} An attention heatmap of the legal clues of a robbery  case with different law charges.}
% \end{figure}
% \begin{figure} [t]   
%     \centering
%     \includegraphics[width = 1\linewidth] {./Figures/case_study_v6.pdf}
%     \caption{\label{fig:7} An attention heatmap of the legal clues of a robbery  case with different law charges.}
% \end{figure}
% \subsection{Contributions of Clues Tracing}
% Extracting the legal clues (i.e., motivation, action, and harm) makes it easier for SEMDR to focus on some core information than directly using the full text of the legal decision for the association measurement.
% Such as the robbery case in Figure \ref{fig:5}, relied on legal clues to calculate the highest rate of association between the crime and the life of the robbery (at 88\%). Exploring the reasons for this further, we find that the description of the crime clearly determines the outcome of the judgement. This is because the offender's actions were theft of property without the controller's attention.
% Figure \ref{fig:6} shows the example of legal clues employed in the interpretation and definition of legal accusation by SEMDR.
% This crime is about theft accusation with the legal judgment is \textbf{(Article 264, theft, 6 months)}. From the criminal fact description, BERT models succeed to figure out expert-defined attributes (e.g. credit card, steal, transfer bank...). However, BERT misjudges it as a credit card fraud accusation under the misleading information of "credit card". TopJudge can predict the relevant article and imprisonment (i.e., article 264, 6 months) and 
% utilize their legal dependencies to predict this charge. Nevertheless, TopJudge still predicts the wrong answer due to the lack of sufficient relevant cases reasoning. Unlike baseline models, SEMDR can extend the training range and provides the correct answer with the guidance of fine-grained analysis of legal clues. 
% To summarize, modeling the semantic representation of legal clues and the reasoning the related criminal cases can significantly help LJP models to solve the problem of predicting conflict.
% \subsection{Case Study}
% Figure 4 shows the example of legal clues employed in the interpretation and definition of legal accusation by SEMDR.
% % In Figure 4, we have shown how SEMDR can help facilitate the performance of charge prediction by choosing a case where it is easy to misjudge. 
% This crime is about theft accusation with the legal judgment is \textbf{(Article 264, theft, 6 months)}. From the criminal fact description, BERT models succeed to figure out expert-defined attributes (e.g. credit card, steal, transfer bank...). However, BERT misjudges it as a credit card fraud accusation under the misleading information of "credit card". TopJudge can predict the relevant article and imprisonment (i.e., article 264, 6 months) and 
% utilize their legal dependencies to predict this charge. Nevertheless, TopJudge still predicts the wrong answer due to the lack of sufficient relevant cases reasoning. Unlike baseline models, SEMDR can extend the training range and provides the correct answer with the guidance of fine-grained analysis of legal clues. 
% To summarize, modeling the semantic representation of legal clues and the reasoning the related criminal cases can significantly help LJP models to solve the problem of predicting conflict.
\section{Conclusion}
% 重申研究目的
% 解释研究成果重要性
% 总结研究成果
% 当前局限性
% 提出建议
This paper has argued that legal judgment prediction (LJP) via a joint semantic enhancement framework. To improve the performance of distinguishing various accusations in different scenarios and avoid the "data hungry" problem in this research field, we propose a novel semantic-aware dual encoder framework, SEMDR. Guided by the ''case enhancement'' strategy, our model can sharpen the differences between confusable accusations and aggregate same-accusation cases to trace legal clues automatically. Specifically, we first build a pre-trained language model for the legal domain based on fine-grained contrastive learning. By applying positive and negative samples, the semantic information of the unknown crime embedding expands significantly. Then, we construct a legal judgment reasoning graph from existing judgment. Experiments on three different scenarios show the accuracy and effectiveness of SEMDR by achieving state-of-the-art performance in the LJP domain. In the future, we will explore the impact of combining other retrieval models to collect more relevant criminal cases to improve performance further.
% \section{Conclusion}
% % 重申研究目的
% % 解释研究成果重要性
% % 总结研究成果
% % 当前局限性
% % 提出建议
% This paper has argued that legal judgment prediction (LJP) via a joint semantic enhancement framework. To improve the performance of distinguishing various accusations in different scenarios and avoid "data hungry" problem in this research field, we propose a novel semantic-aware dual encoder framework, SEMDR. Guided by the ''case annotates case'' strategy, our model can sharpen the differences between confusable accusations and aggregate same-accusation cases to trace legal clues automatically. Specifically, we first built a pre-trained language model for the legal domain based on fine-grained contrastive learning. By applying positive and negative samples, the semantic information of the unknown crime embedding expands significantly. Then, we construct a legal judgment reasoning graph from existing judgment. Experiments on three different scenarios show the accuracy and effectiveness of SEMDR by achieving state-of-the-art performance in LJP domain. In the future, we will explore the impact of combining different retrieval models to collect more relevant criminal cases to further improve prediction performance.
% --(HERE)--
% The insights gained from this study can be concluded as follows, 
% In this paper, we focus on the task of legal judgment prediction (LJP) and address multiple subtasks of judgment predication with a joint learning framework. To be specific, we formalize the criminal clues tracing over these subtasks in a legal judgment knowledge graph, and propose a novel semantic-aware dual encoder framework, SEMDR. To enhance the differences between the various criminal charges through comparative learning methods and to aggregate same-accusation cases to trace legal clues. Under the ''case annotates case'' solution, we have been able to overcome the "data hungry" problem in legal artificial intelligence and improve the accuracy significantly in all subtasks.
% \section{Error Analysis}
% Prediction errors induced by our proposed model can be traced down into the following causes.
% Limited Semantic Information. For the subtasks of law articles and chrages, our model can achieve more than 93\% on accuracy, while under 60\% on the  imprisonment prediction. There are two main reasons for this problem: one is that the distribution of sentencing cases is irregular compared to the first two subtasks, i.e., the results of sentencing for the same crime are highly variable, which poses a non-negligible challenge when aggregating cases, and the other is that the sentencing nodes themselves have very little semantic variability and are very close in spatial distribution after pre-training language model. It also results in sentencing errors.
% Data Imbalance. During the process of case aggregation training, providing LJP nodes with sufficient cases for learning is a prerequisite for accurate prediction, and because of this, when the distribution of cases in the data is unbalanced, it can lead to insufficient training of some nodes, which in turn makes the two models lose their correlation and relevance due to the non-stop understanding of the same classification.
%  \section{Limitations}
%  In this section, the experimental settings  of SEMDR and baseline models are described in detail. Moreover, a serious of experiments are conducted on 5 different real datasets selected from China Artificial Intelligence and Legal Challenges (CAIL2018) and the experimental results are compared and analysed to verify the effectiveness of the semantic-aware combined with knowledge representation learning dual model proposed in this paper.

==> methodology.tex <==
In this section, we introduce the framework of the Semantic-Aware Dual Encoder Model (SEMDR).
\subsection{Preliminary of Legal Judgment Prediction}

Legal Judgment Prediction (LJP) aims to generate the unknown crime's verdicts according to the existing legal judgment documents. It includes three subtasks: \textbf{I}mprisonment prediction, \textbf{C}harge prediction, and Law \textbf{A}rticle prediction. We leverage criminal fact descriptions ($F$) to predict the corresponding judgment instrument labels ($I/C/A$).

\begin{figure}[!t]{
    \centering
 \subfigure[The Standard Format of Legal Judgment Documents.
 ]{    \centering
            \includegraphics[width = 0.75\linewidth]{    
            ./Figures/appendix_v25_a.pdf
            }
            \label{app_a1}
            }
\hfill
  \subfigure[
The Lexicon-Tracing Method in SEMDR.
  ]{
           \includegraphics[width = 0.75\linewidth] {./Figures/appendix_v24_b.pdf}
           \label{app_a2}
            }
    }
    \caption{The Illustration of Fine-Grained Analysis at the Lexicon Level. Figure~\ref{app_a1} shows a standard legal judgment document that can be organized into four sections: statement, date, location, and process. 
    % SEMDR's lexicon-tracing method aims to extract the legal clues in the process section as motivation, action, and harm. 
    Figure~\ref{app_a2} provides an example of applying matching methods in the motivation extraction.}
\end{figure}
\begin{figure}[!t]
    \includegraphics[width = 0.75\linewidth] {./Figures/appendix27.pdf} \caption{The Structure of Some Nodes and Relations in the Legal Judgment Reasoning Graph. 
    % We have defined four types of nodes and six types of relations between criminal cases and corresponding judgment instruments. 
    E.g. $(N_{F1})$\textbf{\color[rgb]{0,0.502,0.502}{-[{Base\_charge\_is}}]-}$(N_{Ca})$ means that the criminal fact crime fact $(N_{F1})$ is judged by the court to have violated the criminal charge $(N_{Ca})$ in our reasoning knowledge graph.}
\label{app_b1}
\end{figure}
SEMDR consists of two modules, including the clue-aware criminal case representation learning module and the multi-evidence enhancement instrument representation learning module. 
We first conduct clue-aware criminal case representations~($H^{F}$) by employing Pre-trained Language Models (PLMs) to encode criminal cases and contrastively training these representations by adding dropout noise~(Sec. \ref{Sec.3.2}).
Then SEMDR establishes a legal judgment reasoning graph to enhance instrument label representation~($\widetilde{H}^{L}$) with the aggregated semantics from criminal cases~(Sec. \ref{Sec.3.3}).

Finally, SEMDR is trained to predict the corresponding instrument label $L_{I/C/A}$ according to criminal fact representation $H^{F}$ using the following loss:
\begin{equation}
\small{\mathcal{L}_{\text{I/C/A}}{=}\mathrm{CrossEntropy}({L_{I/C/A}^\ast}, {{P({L_{I/C/A}|H^{F}})}})},
\end{equation}
where ${P({L_{I/C/A}|H^{F}})}$ denotes the probability to predict correct prediction results ${{L}}$, and ${L^\ast}$ represent the ground truth LJP verification labels. 
${P({L_{I/C/A}|H^{F}})}$ is calculated by the similarity between the representation of 
criminal case~$H^{F}$ and instrument label~$\widetilde{H}_{I/C/A}^{L}$ as:
\begin{equation}
\small{P({L_{I/C/A}|H^{F}})=\mathrm{softmax}({sim(H^{F},\widetilde{H}_{I/C/A}^{L}))}},
\end{equation}
where the ${sim}$ denotes the dot product operation.

\subsection{Clue-Aware Criminal Case Representation}
\label{Sec.3.2}
Based on the research~\cite{haar_sawyer_cummings_1977,lauderdale2012supreme} in the legal field, effective and traceable legal clues can benefit the LJP models to identify confusing cases. As shown in Figure~\ref{app_a1}, There are four sections in a standard legal judgment document, including statement, date, location, and process. To receive more efficient criminal elements, as shown in Figure~\ref{app_a2}, we propose a hybrid approach that combines fuzzy and exact matching techniques to extract lexicon-level legal clues, including motivation, action, and harm, rather than using the full text.
% design a fuzzy and exact matching combination lexicon-tracing methods 
Since legal judgment documents are written in a unique professional format and logical rules, we first delineate the search area for legal clues by template matching in the process section, and then look for pre-defined criminal elements. 
Otherwise, we regard the narrowed area as the legal clue if there is no exact match for the elements.

Given the token sequence of criminal fact in the clue-aware criminal case representation module, we can obtain the corresponding representation of criminal fact~($H^{F}$):
% For the clues tracing, instead of analysing the full description, we extract motivation, action and harm respectively to organize the legal clues from criminal cases.
% 第一版
% \begin{equation}
% \small{\mathrm{Clues}=\{\mathrm{X^{M}, X^{A}, X^{H}}\}},
% \end{equation}
% 第二版
% \begin{equation}
% \small{\mathrm{Clues}=\{\mathrm{X^{Motivation}, X^{Action}, X^{Harm}}\}}.
% \end{equation}
% 第三版
% \begin{equation}
% \small{\mathrm{Clues}=\{\mathrm{X^{Motivation}, X^{Action}, X^{Harm}}\}}.
% \end{equation}
% It can effectively identify and distinguish between similar cases and the specific paradigm of text extraction are presented in the appendix.
% 改版
% where ${\mathrm{X^{M}}},{\mathrm{X^{A}}}$ and ${\mathrm{X^{H}}}$ stand for Motivation, Action and Harm respectively.
% where ${\mathrm{X^{M}}},{\mathrm{X^{A}}}$ and ${\mathrm{X^{H}}}$ stand for Motivation, Action and Harm respectively.
% which include motivation, action, and harm respectively.
% Based on research in the legal field, effective and traceable legal clues can modify the Pre-trained Language Model (PLM) to identify confusing cases and the specific paradigm of text extraction are presented in the appendix.
% 更改位置
% Based on research in the legal field, practical and traceable legal clues can modify the Pre-trained Language Model (PLM) to identify confusing cases, and the details of text extraction paradigm is presented in the appendix.
 % we can obtain the corresponding hidden embedding of criminal fact description~($H^{F}$):
\begin{equation}
\label{hf}
\small{H^{F}=\mathbf{BERT}\{{F^\mathrm{Motivation}, F^\mathrm{Action}, F^\mathrm{Harm}}\}.}
\end{equation} 
% 原版
\begin{figure*}[t]   
    \centering
    \includegraphics[width =\linewidth] {./Figures/fw2_v24.pdf}    
    \caption{The Architecture of SEMDR Framework. We employ lexicon-tracing and sentence representation learning models to strengthen the clue-aware criminal case representations. Then we leverage the multi-case reasoning model to enhance the instrument label representation in the legal judgment reasoning graph.} 
    \label{fig:2}
\end{figure*}
Following previous work~\cite{gao2021simcse}, we add dropout noise to embedding representations and continuously train the criminal case representation $(H^{F}_{i})$ with its positive sample case $(H^{F}_{i})^{+}$ and negative sample case $(H^{F}_{i})^{-}$. The loss function of our contrastive learning~$(\mathcal{L}_{\text{F}})$ is:
% Following previous work~\cite{gao2021simcse}, we add dropout noise to embedding representations and continuously train the criminal case representation ($H^{F}_{i}$) with its positive sample case ($H^{F}_{i}^{+}$) and negative sample case ($H^{F}_{i}^{-}$). The loss function of our contrastive learning~($\mathcal{L}_{\text{F}}$) is:
\begin{equation}
\label{CL}
\small{\mathcal{L}_{\text {F}}=-\log \frac{e^{\operatorname{sim}\left({H}^{F}, H^{F+}_{i}\right) / \tau}}{\sum_{i=1}^{N}\left(e^{\operatorname{sim}\left({H}^{F}, H^{F+}_{i}\right) / \tau}+e^{\operatorname{sim}\left({H}^{F}, H^{F-}_{i}\right) / \tau}\right)}.}
\end{equation}
We randomly sample cases as the negatives during contrastive learning. In addition, the ${sim}$ denotes the cosine similarity operation, and $\tau$ is the temperature hyperparameter.

\subsection{Multi-Evidence Enhancement Instrument Representation} 
% 得有总领，告诉大家后面如何构建的图
% 第一部分是图构建
% 第二部分是graph的初始化 什么当做节点，什么定义为边
% 第三部分是reasoning
\label{Sec.3.3}
To further enhance the representations of judgment instrument labels (${H}^{L}$), we build the legal judgment reasoning graph, 
where we define criminal cases and corresponding instrument labels as nodes, and they are fully connected.
% where each criminal case fact points to the corresponding judgment instruments, and each judgment item is interconnected. 
We apply the continuously trained PLM model in Sec.~\ref{Sec.3.2} to initialize the reasoning graph and update the representation of the legal judgment node ($\widetilde{H}^{L}$) by relevant/similar cases.

\textit{Graph Building.}
% 我们通过case和instrument labels之间的连边放到附录里面 
% and then design relations~(${R}$) to connect these nodes. In addition, the imprisonment node points to its charge node, and both nodes are connected to the law article node. We list all details of nodes and relations definitions in
To explicitly illustrate the association among criminal cases, we define criminal facts and legal instruments as nodes~(${N}$). As shown in Figure~\ref{app_b1}, we also design several relations~(${R}$) to connect these nodes, and then the nodes of instrument labels are also connected internally.

% 问题
\textit{Graph Initialization.}
We first encode the criminal fact $H^{F}$ in Eq.~(\ref{CL}) after contrastive learning and initialize the representation of corresponding criminal fact nodes.

Then we split the judgment instruments of each criminal case into three independent parts: law imprisonment (${L_{I}}$), legal charge (${L_{C}}$), and law article (${L_{A}}$). Similarly, we leverage the BERT to encode the judgment instruments (${H^{L}}$) as:
\begin{equation}
    \small{H_{I/C/A}^{L} = \mathbf{BERT}(L_{{I/C/A}}).}
\end{equation}
These representations can initialize the legal judgment reasoning graph and then be enhanced by more relevant criminal cases.
% In the process of node initialization, we preserve the fact representation $H^{F}$ of each criminal case through the previous PLM (Sec. \ref{Sec.3.2}). 
% For the judgment nodes, including law imprisonment node, law accusation node and law article node, we also exactly take the training embedding from the previous section as the initialization of these nodes.
Besides, SEMDR passes the legal information of connected nodes through criminal cases aggregation, and the relational attention coefficient between nodes can be obtained through an activation function:
\begin{equation} 
\small{{R}_{{ij}}=\mathrm{LeakyReLU}\left({{\omega}}_{{ij}} \cdot [{{N}_{i}} \mid\mid {{N}_{j}}]\right),}
\end{equation}
 where $``\|"$ denotes the concatenation operation of nodes ${{N}_{i}}$ and ${{N}_{j}}$. We then use the dot product to calculate the learnable weight~(${\boldsymbol{{\omega}}_{{ij}}}$) and $\left[ {{N}_{i}} \|  {{N}_{j}}\right]$.

\textit{Multi-Fact Reasoning.} Guided by the relations between cases and corresponding judgment, we leverage the Graph Attention Network (GAT)~\cite{velickovic2018graph} to conduct the graph representation and get the semantic-level attention scores ($\alpha_{i j}$):
\begin{equation}
    \small{\alpha_{{ij}}=\frac{\exp ({R}_{{ij}})}{\sum_{{e} \in \mathcal{O}({i})} \exp ({R}_{{ie}})},}
\end{equation}
where we take a softmax function to normalize the attention score. Moreover, $\mathcal{O}_{i}$ is the set of its 1-hop connected nodes.

Then the updated judgment results representation (${\widetilde{H}^{L}}$) can be enhanced by neighbours with $\alpha$: 
\begin{equation}
 \small{\widetilde{H}^{L}=\sigma\left(\sum_{j \in \mathcal{N}_{i}} \alpha_{i j} \cdot N_{i}\right),}
\end{equation}
where ${\sigma}$ is the ${ELU}$~\cite{clevert2015fast} activation function and 
neighbour nodes (${N_{i}}$) contain both criminal fact nodes and legal judgment nodes within the discovery range.
% the representation is fed into a multi-task learning framework to predict the corresponding verdicts separately.
% neighbour nodes (${N}$) contain both criminal fact and legal judgment nodes within discovery range.
% (${H^L_{I},H^L_{C},H^L_{A}}$)
% $(\{{L_{tp},L_{ac},L_{ra}}\}\subseteq {L})$.
% \begin{equation}
% \small{\{{L_{tp},L_{ac},L_{ra}}\}\subseteq {L}}.}
% \end{equation}
% % ( $\{{L_{tp},L_{ac},L_{ra}}\}\subseteq {L}$ ).
% \textbf{Association calculation.}  Given that SEMDR is a dual model, we perform the dot product operation on the two independently encoded vectors ($H^{F}_{i}, H^{L}_{i}$) and select the highest score $({S_{i})$ as final results from candidate answers. The prediction probability ${P({L|H^{F}_{i}})}$ between the criminal fact representation ${H^{F}_{i}}$ and the prediction label ${H^{L}_{i}}$:
% \begin{equation}
% \small{S_{i}=\mathrm{Linear}(H^{F}_{i} \cdot H^{L}_{i}),}
% \end{equation}
% \begin{equation}
%     \small{{{P({L|H^{F}_{i}})}}=\mathrm{softmax}(S_{i}).}
% \end{equation}
% \textbf{Loss Function.} 
% Finally, the formulation of the cross-entropy-based loss $\mathcal{L}_{C}$ cross the dual framework can be derived as:
% \begin{equation}
% \small{\mathcal{L}_{C}{=}\mathrm{CrossEntropy}(\mathrm{L^\ast}, {{P({L|H^{F}_{i}})}}),}
% \end{equation}
% where $\mathrm{L^\ast}$ represents the ground truth LJP verification label set. Specifically, the label will be set to 1 only when the prediction is correct, and conversely, the label is set to 0 if the prediction is wrong.
% we will employ the dot product to calculate the association probability ${P({L|H^{F},G})}$ between the criminal fact representation ${H^{F}}$ and the prediction label ${Z^{L}$:
% \begin{equation}
%     \small{S^{L}=\mathrm{Linear}(H^{F} \cdot Z^{L}).}
% \end{equation}
% \begin{equation}
%     \small{{P({L|H^{F},G})}=\mathrm{softmax_{L}}((S^{L})).}
% \end{equation}
% \textbf{Loss Function.} Given that SEMDR is a dual model, we perform the dot product operation on the two independently encoded vectors ($H^{F}, L$) and select the verdict with the highest score as final prediction $H^{L}$ from candidate answers. Then the formulation of the cross-entropy-based loss $\mathcal{L}_{C}$ cross the dual framework can be derived as shown:
% \begin{equation}
% \small{\mathcal{L}_{C}{=}\mathrm{CrossEntropy} ( L, \mathrm{softmax}(\hat{L} \cdot H^{F})),}
% \end{equation}
% where the categories of criminal fact description $H^{F}$ and legal Judgment Prediction (LJP) label $L$ are $n$ and $m$ respectively.
% \begin{equation}
%  \small{\left(\left\{{L}_{ac}},{L}_{ra}},{L}_{tp}\right\}\subseteq {\{L\}}\right).}
% \end{equation}
% Besides, as illustration in Figure 2, we have defined two categories of relations (${R}_{}^{fl},{R}_{}^{ll} \in \left\{{R}\right\}$) 
% among different criminal cases and obtained the corresponding triple data ($\left{T}_{fl},{T}_{ll} \in \left\{{T}\right\}\right$) as follows:

% \begin{equation}
% \small{{T}_{f l}= (  \mathrm{F}_{\mathrm{i}}, {R}_{i j}^{f l} ,\space {L}_{{j}}); {T}_{l l}=(  {L}_{{i}}, {R}_{i j}^{l l} ,\space {L}_{{j}} ).}
% \end{equation}

% Guide by the relations {\{R\}} between crimes and their corresponding judgment results, we can apply the Graph Attention Network (GAT)~\cite{velickovic2018graph} to derive the graph representation and the attention scores $\alpha_{i j}$:
%  \begin{equation}
%   \small{\alpha_{i j}=\frac{\exp \left(\overrightarrow{\mathbf{a}}^{T}\left[H^{E}_{i}\left\|H^{R}_{ij}\right\| H^{E}_{j}\right]\right)}{\sum_{j \in \mathcal{N}_{i}} \exp \left(\overrightarrow{\mathbf{a}}^{T}\left[H^{E}_{i}\left\|H^{R}_{ij}\right\| H^{E}_{j}\right]\right)},}
% \end{equation}

% \subsection{Supervised Contrastive Learning}
% % 引出对比学习结合的PLM(主要是SimCSE)
% Since most of the trial documents in CAIL2018 are in Chinese, we adopt a pre-trained BERT~\cite{BERT-2019} as the sentence encoder module. Given an token sequence \{$x_{i}$\} as input to the encoder module to obtain the hidden representation of criminal fact description $H^{F}$:

% \begin{small}
% \begin{equation}
% H^{F}=\{[\mathrm{CLS}]x_{1}, x_{2}, \ldots, x_{n}[\mathrm{SEP}]\}_\mathrm{[CLS]},
% \end{equation}
% \end{small}
% For the criminal clues tracing, we have adopted a semantic-aware PLM to enhance the comprehension of factual elements, including criminal actions, criminal harm and motivations. Specifically, each hidden representation $H^{F}_{i}$ will be compared with its positive sample group $ H^{F}_{i}^{+}$ and negative sample group $H^{F}_{j}^{-}$ during contrastive learning. The formulation of criminal fact description loss $\mathcal{L}_{\text {F}}$ is:

% \begin{equation}
% \small{\mathcal{L}_{\text {F}}= -\log \frac{e^{\mathrm{sim}({H}^{F}_{i}, {H}^{F}_{i}^{+}) / \tau}}{\sum_{j=1}^{N}(e^{\mathrm{sim}(H_{i}^{F}, H_{j}^{F}^{+}) / \tau}+e^{\mathrm{sim}(H_{i}^{F}, H_{j}^{F}^{-}) / \tau})},}
% \end{equation}
% where $\mathrm{sim}(H^{F}_{i}, H^{F}_{j})$ is the cosine similarity operation $\frac{{H^{F}_{i}} {H}^{F}_{j}}{\left\|{H}^{F}_{i}\right\|\cdot \left\|\mathrm{H}^{F}_{j}\right\|}$ and $\tau$ is the temperature hyperparameter that regulates sensitivity of the model.

% \subsection{Case Enhancement on Reasoning Graph} 
% \textbf{Nodes and Edges Initialization.}
% % We model the knowledge of criminal case enhancement with a customized knowledge graph. In the process of node initialization, we leverage the previous CL-based PLM to obtain corresponding node embedding of fact set $(F)$, judgment label set $(L)$ and relation edge set $(R)$ from each instance criminal case.
% We model the knowledge of criminal case enhancement with a customized knowledge graph. In the process of node initialization, we leverage the previous (in equation 5) CL-based PLM to obtain corresponding node $E$ embedding representation $H^{E}$ (including criminal fact set $F$, legal judgment label set $L$) and relation edge representation $H^{R}$ from each instance criminal case:

% \begin{small}
% \begin{equation}
% H^{E}_{i}}=\mathbf{PLM}\left \{{E}_{i}\right \}; H^{R}_{ij}} = \mathbf{PLM}\left \{{R}_{ij}\right \}.
% \end{equation}
% \end{small}
% \textbf{Reasoning with Existing Criminal Cases.} After the initialisation of the nodes and relations on the legal judgment knowledge graph $(G)$, SEMDR will reasoning the legal clues from relevant criminal case. 
% Guide by the relations {\{R\}} between crimes and their corresponding judgment results, we can apply the Graph Attention Network (GAT)~\cite{velickovic2018graph} to derive the graph representation and the attention scores $\alpha_{i j}$:

% \begin{small}
%  \begin{equation}
%   \alpha_{i j}=\frac{\exp \left(\overrightarrow{\mathbf{a}}^{T}\left[H^{E}_{i}\left\|H^{R}_{ij}\right\| H^{E}_{j}\right]\right)}{\sum_{j \in \mathcal{N}_{i}} \exp \left(\overrightarrow{\mathbf{a}}^{T}\left[H^{E}_{i}\left\|H^{R}_{ij}\right\| H^{E}_{j}\right]\right)},
% \end{equation}
% \end{small}
% % \begin{equation}
% %     EGAT: |\mathbf E_{i} \| \mathbf E_{k}|\Rightarrow |\mathbf E_{i} \|R_{ij}\| \mathbf E_{k}|
% % \end{equation}
% where $\|$ denotes the concatenation operation of two connected nodes $E_{i}$, $ E_{j}$ with their relation $R_{ij}$. We then take a dot product on the learnable weight vector \overrightarrow{\boldsymbol{a}}^{T}$ and $[H^{E}_{i}\left\|H^{R}_{ij}\right\| H^{E}_{j}]$. Moreover, $\mathcal{N}_{i}$ is the set of its one-hop neighbours and a softmax layer is applied to normalize the attention scores on each node’s incoming edges. 
% The updated entity node representation ${H^{E}_{i}}^{\prime}$ will be aggregated by the neighbour nodes with the attention scores: 

% \begin{small}
% \begin{equation}
%   {H^{E}_{i}}^{\prime}=\sigma\left(\sum_{j \in \mathcal{N}_{i}} \alpha_{i j}\cdot {W} \cdot {H^{E}_{i}}\right),
% \end{equation}
% \end{small}
% where and ${\sigma}$ is a activation function. Finally, we will employ the dot product to calculate the association probability ${P({L|H^{F},G})}$ between the criminal fact representation ${H^{F}}$ and the prediction label ${H^{L}$:
% \begin{equation}
%     \small{S^{L}=\mathrm{softmax}(H^{F} \cdot H^{L}),}
% \end{equation}
% \begin{equation}
%     \small{{P({L|H^{F},G})}=\mathrm{softmax_{L}}(\mathrm{Linear}(S^{L})).}
% \end{equation}
% \textbf{Loss Function.} Given that SEMDR is a dual model, we perform the dot product operation on the two independently encoded vectors ($H^{F}, L$) and select the verdict with the highest score as final prediction $H^{L}$ from candidate answers. Then the formulation of the cross-entropy-based loss $\mathcal{L}_{C}$ spanning the dual framework can be derived as shown:
% \begin{equation}
% \small{\mathcal{L}_{C}{=}\mathrm{CrossEntropy} ( L, \mathrm{softmax}(\hat{L} \cdot H^{F})),}
% \end{equation}
% where the categories of criminal fact description $H^{F}$ and legal Judgment Prediction (LJP) label $L$ are $n$ and $m$ respectively.
% Then the loss function of a node on the graph can be denoted as:
% \begin{equation}
%     \mathcal{L}_{\text {
%     Node}}= {\textstyle \sum_{i}^{n+m}} (E_{i} - E_{i}^{\prime})
% \end{equation}

% \textbf{Knowledge Representation Learning.} After the initialisation of the nodes and relations on the legal judgment knowledge graph $(G)$, SEMDR will train the triple set $\left\{{T}\right\}\right$ as shown in the equation (2), (3). Specifically, SimplE~\cite{kazemi2018simple} is a similarity-based Knowledge Representation Learning (KRL) algorithm that can collect more associations among various 
% criminal nodes and judgment result nodes. SimplE score function can be expressed as followed:
% \begin{equation}
% % \text { score }\left(\text { Triplet }_{fl}\right)=\sum_{j\in {N}_{i}}\left(E_{i} * \mathrm{R}_{fl_{(ij}} * \mathrm{E}_{j}\right) 
% \text { score }\left(\text { T}\right)= \frac{{ T }(\oplus )+{ T }(\ominus )}{2} 
% \end{equation}

% \begin{equation}
% {T}(\oplus)=\sum_{j\in {N}_{i}}\left(E_{i} \cdot   \mathrm{R}_{ij}^{+} \cdot   \mathrm{E}_{j}\right)
% \end{equation}
% \begin{equation}
%     {T}(\ominus)=\sum_{j\in {N}_{i}}\left(E_{i} \cdot \mathrm{R}_{ij}^{-} \cdot \mathrm{E}_{j}\right)
% \end{equation}

% Where ${R}_{{ij}}^{+}$ is the forward relation from head entities to tail entities, while ${R}_{ij}^{-}$ is the corresponding inverse relation on the opposite direction. According to the real-world situation, ${T}(\oplus )$ can be treated as the positive triple group and ${T}(\ominus )$ is the negative triple group respectively. Thus, we can derive the loss function ${\mathcal{L}_{\text {Triple}}$ of the triple data $T$ during KRL as followed:

% % and it also means that $(E_{i}, {R}_{(fl)_{ij}}^{+}, E_{j})\in G,(E_{i}. {R}_{(fl)_{i j}}^{-},E_{j})\notin G$.
% % Similarly, we can obtain the score fucntion of $\mathrm{T }_{ll}\right)$:
% % \begin{equation}
% % \operatorname{score}\left(T_{l l}\right)=\frac{T_{l l}(\oplus)+T_{l l}(\ominus)}{2}
% % \end{equation}



%   \begin{equation}
% \mathcal{L}_{T r i p l e}=\sum_{T\in G} \operatorname{softplus}\left(-l \cdot Score(T)\right)+\lambda\|\theta \|_{2}^{2}
%  \end{equation}
%   \begin{equation}
% \mathit{{softplus}} (x)=\log (1+\exp (x))
%  \end{equation}
 
%  Where $T$ contains two types of designed triple shown in preliminaries. ${l}\in \left \{ -1,1 \right \} $ represents the label of a triple, ${1}$ stands for the positive triples and negatives represent as ${-1}$. ${\lambda}$ is the regularization hyperparameter and ${\theta}$ represents the parameters of the model. Finally, we can generalize the loss function of the legal judgment knowledge graph ${(G)}$, which contains the loss of criminal case aggregation and the loss of triplet data during KRL.
%  \begin{equation}
%  \mathcal{L}_{\text {Graph}}= \mathcal{L}_{\text {Node}} +\mathcal{L}_{\text {Triplet}}
%   \end{equation}

%  \begin{equation}
%  \mathcal{L}=\sum_{T \in {G}} \log (1+\exp (-S(T)))+\sum_{T^{\prime} \notin {G}} \log \left(1+\exp \left(S\left(T^{\prime}\right)\right)\right)
%  \end{equation}
 
% \textbf{Graph Attention Networks.} Guide by the relations {\{R\}} between crimes and their judgment results, we can obtain the adjacency matrix $\mathcal{G} \in \mathbb{R}^{(m+n) \times(m+n)}$. Then we apply the Graph Attention Network (GAT)~\cite{velickovic2018graph} to derive the graph representation and the attention scores $\alpha_{i j}$.
% %  \begin{equation}
% % \boldsymbol{G}=f(\operatorname{GAT}(\boldsymbol{E} ; \mathcal{G}))
% % \end{equation}
%  \begin{equation}
%   \alpha_{i j}=\frac{\exp \left(\overrightarrow{\mathbf{a}}^{T}\left[\mathbf E_{i} \| \mathbf E_{j}\right]\right)}{\sum_{k \in \mathcal{N}_{i}} \exp \left(\overrightarrow{\mathbf{a}}^{T}\left[\mathbf E_{i} \| \mathbf E_{k}\right]\right)}
% \end{equation}

% During this operation, we combine the embedding of the two connected nodes $\mathbf E_{i},\mathbf E_{j}$, where $\|$ denotes concatenation. We dot product of a learnable weight vector $\overrightarrow{\boldsymbol{a}}^{(T)}$ and $\left[\mathbf E_{i} \| \mathbf E_{j}\right]$. Moreover, in equation (8), $\mathcal{N}(i)$ is the set of its one-hop neighbours and a softmax layer is applied to normalize the attention scores on each node’s incoming edges. 
% The entity nodes $E^{\prime}$ will be updated by the embedding from neighbours are aggregated together and scaled by the attention scores as followed: 
% \begin{equation}
%   E^{\prime}=\sigma\left(\sum_{j \in \mathcal{N}_{i}} \alpha_{i j}\cdot {W} \cdot E\right)
% \end{equation}

% Where ${W}$ is a learnable weight matrix and the final entity nodes will be applied to predict the judgment results across two independent models. The loss function of a node on the graph can be denoted as:
% \begin{equation}
%     \mathcal{L}_{\text {
%     Node}}= {\textstyle \sum_{i}^{n+m}} (E_{i} - E_{i}^{\prime})
% \end{equation}

% \textbf{Knowledge Representation Learning.} Meanwhile,  our model encodes the triplet set $\left\{\mathbf{T}\right\}\right$ as shown in the equation (2), (3). SimplE~\cite{kazemi2018simple} is a similarity-based Knowledge Representation Learning (KRL) algorithm that can collect more associations among various crimes nodes and judgment result nodes in the legal judgment knowlesge graph. The score fucntion of ${T}_{fl}\right)$ shown as followed:
% \begin{equation}
% % \text { score }\left(\text { Triplet }_{fl}\right)=\sum_{j\in {N}_{i}}\left(E_{i} * \mathrm{R}_{fl_{(ij}} * \mathrm{E}_{j}\right) 
% \text { score }\left(\text { T}_{fl}\right)= \frac{{ T }_{fl}(\oplus )+{ T }_{fl}(\ominus )}{2} 
% \end{equation}

% \begin{equation}
% { T  }_{fl}(\oplus)=\sum_{j\in {N}_{i}}\left(F_{i} \cdot   \mathrm{R}_{ij}^{fl+} \cdot   \mathrm{L}_{j}\right)
% \end{equation}
% \begin{equation}
%     { T  }_{fl}(\ominus)=\sum_{j\in {N}_{i}}\left(F_{i} \cdot \mathrm{R}_{ij}^{fl-} \cdot \mathrm{L}_{j}\right)
% \end{equation}

% Where ${ T }_{fl}(\oplus )$ is the positive triplet group and ${ T }_{fl}(\ominus )$ is the negative triplet group respectively, and it also means that $(E_{i}, {R}_{(fl)_{ij}}^{+}, E_{j})\in G,(E_{i}. {R}_{(fl)_{i j}}^{-},E_{j})\notin G$. Similarly, we can obtain the score fucntion of $\mathrm{T }_{ll}\right)$ in equation (3):

% \begin{equation}
% % \text { score }\left(\text { Triplet }_{fl}\right)=\sum_{j\in {N}_{i}}\left(E_{i} * \mathrm{R}_{fl_{(ij}} * \mathrm{E}_{j}\right) 
% \text { score }\left(\text { T  }_{ll}\right)= \frac{{ T  }_{ll}(\oplus )+{ T  }_{ll}(\ominus )}{2} 
% \end{equation}
% % \begin{equation}
% % { Triplet }_{fl}(\oplus )=\sum_{j\in {N}_{i}}\left(E_{i} * \mathrm{R}_{(fl)_{i j}} * \mathrm{E}_{j}\right)    
% % \end{equation}
% % \begin{equation}
% %     { Triplet }_{fl}(\ominus)=\sum_{j\in {N}_{i}}\left(E_{i} * \mathrm{R}_{(fl)_{i j}}{}^{inv} * \mathrm{E}_{j}\right)
% % \end{equation}

% Thus, we can generalize the loss function of the legal judgment knowledge graph, which contains the loss of criminal case aggregation and the loss of triplet data during KRL.
%  \begin{equation}
%  \mathcal{L}_{\text {Graph}}= \mathcal{L}_{\text {Node}} +\mathcal{L}_{\text {Triplet}}
%   \end{equation}
%  \begin{equation}
%  \mathcal{L}=\sum_{T \in {G}} \log (1+\exp (-S(T)))+\sum_{T^{\prime} \notin {G}} \log \left(1+\exp \left(S\left(T^{\prime}\right)\right)\right)
%  \end{equation}
 
%   \begin{equation}
%  \mathcal{L}=\sum_{T \in {G}} \mathit { softplus }(-l \cdot \text { T})+\lambda\|\theta\|_{2}^{2}
%  \end{equation}
 
%   \begin{equation}
% \mathit{{softplus}} (x)=\log (1+\exp (x))
%  \end{equation}



